An Algebraic Glimpse at Bunched Implications and Separation Logic

We overview the logic of Bunched Implications (BI) and Separation Logic (SL) from a perspective inspired by Hiroakira Ono's algebraic approach to substructural logics. We propose generalized BI algebras (GBI-algebras) as a common framework for algebras arising via "declarative resource reading", intuitionistic generalizations of relation algebras and arrow logics and the distributive Lambek calculus with intuitionistic implication. Apart from existing models of BI (in particular, heap models and effect algebras), we also cover models arising from weakening relations, formal languages or more fine-grained treatment of labelled trees and semistructured data. After briefly discussing the lattice of subvarieties of GBI, we present a suitable duality for GBI along the lines of Esakia and Priestley and an algebraic proof of cut elimination in the setting of residuated frames of Galatos and Jipsen. We also show how the algebraic approach allows generic results on decidability, both positive and negative ones. In the final part of the paper, we gently introduce the substructural audience to some theory behind state-of-art tools, culminating with an algebraic and proof-theoretic presentation of (bi-)abduction.

==> mathpartir.tex <==
%  Mathpartir --- Math Paragraph for Typesetting Inference Rules
%
%  Copyright (C) 2001, 2002, 2003, 2004, 2005 Didier Rémy
%
%  Author         : Didier Remy 
%  Version        : 1.2.0
%  Bug Reports    : to author
%  Web Site       : http://pauillac.inria.fr/~remy/latex/
% 
%  Mathpartir is free software; you can redistribute it and/or modify
%  it under the terms of the GNU General Public License as published by
%  the Free Software Foundation; either version 2, or (at your option)
%  any later version.
%  
%  Mathpartir is distributed in the hope that it will be useful,
%  but WITHOUT ANY WARRANTY; without even the implied warranty of
%  MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%  GNU General Public License for more details 
%  (http://pauillac.inria.fr/~remy/license/GPL).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  File mathpartir.sty (LaTeX macros)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{mathpartir}
    [2005/12/20 version 1.2.0 Math Paragraph for Typesetting Inference Rules]

%%

%% Identification
%% Preliminary declarations

\RequirePackage {keyval}

%% Options
%% More declarations

%% PART I: Typesetting maths in paragraphe mode

%% \newdimen \mpr@tmpdim
%% Dimens are a precious ressource. Uses seems to be local.
\let \mpr@tmpdim \@tempdima

% To ensure hevea \hva compatibility, \hva should expands to nothing 
% in mathpar or in inferrule
\let \mpr@hva \empty

%% normal paragraph parametters, should rather be taken dynamically
\def \mpr@savepar {%
  \edef \MathparNormalpar
     {\noexpand \lineskiplimit \the\lineskiplimit
      \noexpand \lineskip \the\lineskip}%
  }

\def \mpr@rulelineskip {\lineskiplimit=0.3em\lineskip=0.2em plus 0.1em}
\def \mpr@lesslineskip {\lineskiplimit=0.6em\lineskip=0.5em plus 0.2em}
\def \mpr@lineskip  {\lineskiplimit=1.2em\lineskip=1.2em plus 0.2em}
\let \MathparLineskip \mpr@lineskip
\def \mpr@paroptions {\MathparLineskip}
\let \mpr@prebindings \relax

\newskip \mpr@andskip \mpr@andskip 2em plus 0.5fil minus 0.5em

\def \mpr@goodbreakand
   {\hskip -\mpr@andskip  \penalty -1000\hskip \mpr@andskip}
\def \mpr@and {\hskip \mpr@andskip}
\def \mpr@andcr {\penalty 50\mpr@and}
\def \mpr@cr {\penalty -10000\mpr@and}
\def \mpr@eqno #1{\mpr@andcr #1\hskip 0em plus -1fil \penalty 10}

\def \mpr@bindings {%
  \let \and \mpr@andcr
  \let \par \mpr@andcr
  \let \\\mpr@cr
  \let \eqno \mpr@eqno
  \let \hva \mpr@hva
  } 
\let \MathparBindings \mpr@bindings

% \@ifundefined {ignorespacesafterend}
%    {\def \ignorespacesafterend {\aftergroup \ignorespaces}

\newenvironment{mathpar}[1][]
  {$$\mpr@savepar \parskip 0em \hsize \linewidth \centering
     \vbox \bgroup \mpr@prebindings \mpr@paroptions #1\ifmmode $\else
     \noindent $\displaystyle\fi
     \MathparBindings}
  {\unskip \ifmmode $\fi\egroup $$\ignorespacesafterend}

\newenvironment{mathparpagebreakable}[1][]
  {\begingroup 
   \par
   \mpr@savepar \parskip 0em \hsize \linewidth \centering
      \mpr@prebindings \mpr@paroptions #1%
      \vskip \abovedisplayskip \vskip -\lineskip%
     \ifmmode  \else  $\displaystyle\fi
     \MathparBindings
  }
  {\unskip
   \ifmmode $\fi \par\endgroup
   \vskip \belowdisplayskip
   \noindent
  \ignorespacesafterend}

% \def \math@mathpar #1{\setbox0 \hbox {$\displaystyle #1$}\ifnum
%     \wd0 < \hsize  $$\box0$$\else \bmathpar #1\emathpar \fi}

%%% HOV BOXES

\def \mathvbox@ #1{\hbox \bgroup \mpr@normallineskip 
  \vbox \bgroup \tabskip 0em \let \\ \cr
  \halign \bgroup \hfil $##$\hfil\cr #1\crcr \egroup \egroup
  \egroup}

\def \mathhvbox@ #1{\setbox0 \hbox {\let \\\qquad $#1$}\ifnum \wd0 < \hsize
      \box0\else \mathvbox {#1}\fi}


%% Part II -- operations on lists

\newtoks \mpr@lista
\newtoks \mpr@listb

\long \def\mpr@cons #1\mpr@to#2{\mpr@lista {\\{#1}}\mpr@listb \expandafter
{#2}\edef #2{\the \mpr@lista \the \mpr@listb}}

\long \def\mpr@snoc #1\mpr@to#2{\mpr@lista {\\{#1}}\mpr@listb \expandafter
{#2}\edef #2{\the \mpr@listb\the\mpr@lista}}

\long \def \mpr@concat#1=#2\mpr@to#3{\mpr@lista \expandafter {#2}\mpr@listb
\expandafter {#3}\edef #1{\the \mpr@listb\the\mpr@lista}}

\def \mpr@head #1\mpr@to #2{\expandafter \mpr@head@ #1\mpr@head@ #1#2}
\long \def \mpr@head@ #1#2\mpr@head@ #3#4{\def #4{#1}\def#3{#2}}

\def \mpr@flatten #1\mpr@to #2{\expandafter \mpr@flatten@ #1\mpr@flatten@ #1#2}
\long \def \mpr@flatten@ \\#1\\#2\mpr@flatten@ #3#4{\def #4{#1}\def #3{\\#2}}

\def \mpr@makelist #1\mpr@to #2{\def \mpr@all {#1}%
   \mpr@lista {\\}\mpr@listb \expandafter {\mpr@all}\edef \mpr@all {\the
   \mpr@lista \the \mpr@listb \the \mpr@lista}\let #2\empty 
   \def \mpr@stripof ##1##2\mpr@stripend{\def \mpr@stripped{##2}}\loop
     \mpr@flatten \mpr@all \mpr@to \mpr@one
     \expandafter \mpr@snoc \mpr@one \mpr@to #2\expandafter \mpr@stripof
     \mpr@all \mpr@stripend  
     \ifx \mpr@stripped \empty \let \mpr@isempty 0\else \let \mpr@isempty 1\fi
     \ifx 1\mpr@isempty
   \repeat
}

\def \mpr@rev #1\mpr@to #2{\let \mpr@tmp \empty
   \def \\##1{\mpr@cons ##1\mpr@to \mpr@tmp}#1\let #2\mpr@tmp}

%% Part III -- Type inference rules

\newif \if@premisse
\newbox \mpr@hlist
\newbox \mpr@vlist
\newif \ifmpr@center \mpr@centertrue
\def \mpr@htovlist {%
   \setbox \mpr@hlist
      \hbox {\strut
             \ifmpr@center \hskip -0.5\wd\mpr@hlist\fi
             \unhbox \mpr@hlist}%
   \setbox \mpr@vlist
      \vbox {\if@premisse  \box \mpr@hlist \unvbox \mpr@vlist
             \else \unvbox \mpr@vlist \box \mpr@hlist
             \fi}%
}
% OLD version
% \def \mpr@htovlist {%
%    \setbox \mpr@hlist
%       \hbox {\strut \hskip -0.5\wd\mpr@hlist \unhbox \mpr@hlist}%
%    \setbox \mpr@vlist
%       \vbox {\if@premisse  \box \mpr@hlist \unvbox \mpr@vlist
%              \else \unvbox \mpr@vlist \box \mpr@hlist
%              \fi}%
% }

\def \mpr@item #1{$\displaystyle #1$}
\def \mpr@sep{2em}
\def \mpr@blank { }
\def \mpr@hovbox #1#2{\hbox
  \bgroup
  \ifx #1T\@premissetrue
  \else \ifx #1B\@premissefalse
  \else
     \PackageError{mathpartir}
       {Premisse orientation should either be T or B}
       {Fatal error in Package}%
  \fi \fi
  \def \@test {#2}\ifx \@test \mpr@blank\else
  \setbox \mpr@hlist \hbox {}%
  \setbox \mpr@vlist \vbox {}%
  \if@premisse \let \snoc \mpr@cons \else \let \snoc \mpr@snoc \fi
  \let \@hvlist \empty \let \@rev \empty
  \mpr@tmpdim 0em
  \expandafter \mpr@makelist #2\mpr@to \mpr@flat
  \if@premisse \mpr@rev \mpr@flat \mpr@to \@rev \else \let \@rev \mpr@flat \fi
  \def \\##1{%
     \def \@test {##1}\ifx \@test \empty
        \mpr@htovlist
        \mpr@tmpdim 0em %%% last bug fix not extensively checked
     \else
      \setbox0 \hbox{\mpr@item {##1}}\relax
      \advance \mpr@tmpdim by \wd0
      %\mpr@tmpdim 1.02\mpr@tmpdim
      \ifnum \mpr@tmpdim < \hsize
         \ifnum \wd\mpr@hlist > 0
           \if@premisse
             \setbox \mpr@hlist 
                \hbox {\unhbox0 \hskip \mpr@sep \unhbox \mpr@hlist}%
           \else
             \setbox \mpr@hlist
                \hbox {\unhbox \mpr@hlist  \hskip \mpr@sep \unhbox0}%
           \fi
         \else 
         \setbox \mpr@hlist \hbox {\unhbox0}%
         \fi
      \else
         \ifnum \wd \mpr@hlist > 0
            \mpr@htovlist 
            \mpr@tmpdim \wd0
         \fi
         \setbox \mpr@hlist \hbox {\unhbox0}%
      \fi
      \advance \mpr@tmpdim by \mpr@sep
   \fi
   }%
   \@rev
   \mpr@htovlist
   \ifmpr@center \hskip \wd\mpr@vlist\fi \box \mpr@vlist
   \fi
   \egroup
}

%%% INFERENCE RULES

\@ifundefined{@@over}{%
    \let\@@over\over % fallback if amsmath is not loaded
    \let\@@overwithdelims\overwithdelims
    \let\@@atop\atop \let\@@atopwithdelims\atopwithdelims
    \let\@@above\above \let\@@abovewithdelims\abovewithdelims
  }{}

%% The default

\def \mpr@@fraction #1#2{\hbox {\advance \hsize by -0.5em
    $\displaystyle {#1\mpr@over #2}$}}
\def \mpr@@nofraction #1#2{\hbox {\advance \hsize by -0.5em
    $\displaystyle {#1\@@atop #2}$}}

\let \mpr@fraction \mpr@@fraction

%% A generic solution to arrow

\def \mpr@make@fraction #1#2#3#4#5{\hbox {%
     \def \mpr@tail{#1}%
     \def \mpr@body{#2}%
     \def \mpr@head{#3}%
     \setbox1=\hbox{$#4$}\setbox2=\hbox{$#5$}%
     \setbox3=\hbox{$\mkern -3mu\mpr@body\mkern -3mu$}%
     \setbox3=\hbox{$\mkern -3mu \mpr@body\mkern -3mu$}%
     \dimen0=\dp1\advance\dimen0 by \ht3\relax\dp1\dimen0\relax
     \dimen0=\ht2\advance\dimen0 by \dp3\relax\ht2\dimen0\relax
     \setbox0=\hbox {$\box1 \@@atop \box2$}%
     \dimen0=\wd0\box0
     \box0 \hskip -\dimen0\relax
     \hbox to \dimen0 {$%
       \mathrel{\mpr@tail}\joinrel
       \xleaders\hbox{\copy3}\hfil\joinrel\mathrel{\mpr@head}%
     $}}}

%% Old stuff should be removed in next version
\def \mpr@@nothing #1#2
    {$\lower 0.01pt \mpr@@nofraction {#1}{#2}$}
\def \mpr@@reduce #1#2{\hbox
    {$\lower 0.01pt \mpr@@fraction {#1}{#2}\mkern -15mu\rightarrow$}}
\def \mpr@@rewrite #1#2#3{\hbox
    {$\lower 0.01pt \mpr@@fraction {#2}{#3}\mkern -8mu#1$}}
\def \mpr@infercenter #1{\vcenter {\mpr@hovbox{T}{#1}}}

\def \mpr@empty {}
\def \mpr@inferrule
  {\bgroup
     \ifnum \linewidth<\hsize \hsize \linewidth\fi
     \mpr@rulelineskip
     \let \and \qquad
     \let \hva \mpr@hva
     \let \@rulename \mpr@empty
     \let \@rule@options \mpr@empty
     \let \mpr@over \@@over
     \mpr@inferrule@}
\newcommand {\mpr@inferrule@}[3][]
  {\everymath={\displaystyle}%       
   \def \@test {#2}\ifx \empty \@test
      \setbox0 \hbox {$\vcenter {\mpr@hovbox{B}{#3}}$}%
   \else 
   \def \@test {#3}\ifx \empty \@test
      \setbox0 \hbox {$\vcenter {\mpr@hovbox{T}{#2}}$}%
   \else
   \setbox0 \mpr@fraction {\mpr@hovbox{T}{#2}}{\mpr@hovbox{B}{#3}}%
   \fi \fi
   \def \@test {#1}\ifx \@test\empty \box0
   \else \vbox 
%%% Suggestion de Francois pour les etiquettes longues
%%%   {\hbox to \wd0 {\RefTirName {#1}\hfil}\box0}\fi
      {\hbox {\RefTirName {#1}}\box0}\fi
   \egroup}

\def \mpr@vdotfil #1{\vbox to #1{\leaders \hbox{$\cdot$} \vfil}}

% They are two forms
% \inferrule [label]{[premisses}{conclusions}
% or
% \inferrule* [options]{[premisses}{conclusions}
%
% Premisses and conclusions are lists of elements separated by \\
% Each \\ produces a break, attempting horizontal breaks if possible, 
% and  vertical breaks if needed. 
% 
% An empty element obtained by \\\\ produces a vertical break in all cases. 
%
% The former rule is aligned on the fraction bar. 
% The optional label appears on top of the rule
% The second form to be used in a derivation tree is aligned on the last
% line of its conclusion
% 
% The second form can be parameterized, using the key=val interface. The
% folloiwng keys are recognized:
%       
%  width                set the width of the rule to val
%  narrower             set the width of the rule to val\hsize
%  before               execute val at the beginning/left
%  lab                  put a label [Val] on top of the rule
%  lskip                add negative skip on the right
%  left                 put a left label [Val]
%  Left                 put a left label [Val],  ignoring its width 
%  right                put a right label [Val]
%  Right                put a right label [Val], ignoring its width
%  leftskip             skip negative space on the left-hand side
%  rightskip            skip negative space on the right-hand side
%  vdots                lift the rule by val and fill vertical space with dots
%  after                execute val at the end/right
%  
%  Note that most options must come in this order to avoid strange
%  typesetting (in particular  leftskip must preceed left and Left and
%  rightskip must follow Right or right; vdots must come last 
%  or be only followed by rightskip. 
%  

%% Keys that make sence in all kinds of rules
\def \mprset #1{\setkeys{mprset}{#1}}
\define@key {mprset}{andskip}[]{\mpr@andskip=#1}
\define@key {mprset}{lineskip}[]{\lineskip=#1}
\define@key {mprset}{flushleft}[]{\mpr@centerfalse}
\define@key {mprset}{center}[]{\mpr@centertrue}
\define@key {mprset}{rewrite}[]{\let \mpr@fraction \mpr@@rewrite}
\define@key {mprset}{atop}[]{\let \mpr@fraction \mpr@@nofraction}
\define@key {mprset}{myfraction}[]{\let \mpr@fraction #1}
\define@key {mprset}{fraction}[]{\def \mpr@fraction {\mpr@make@fraction #1}}
\define@key {mprset}{sep}{\def\mpr@sep{#1}}

\newbox \mpr@right
\define@key {mpr}{flushleft}[]{\mpr@centerfalse}
\define@key {mpr}{center}[]{\mpr@centertrue}
\define@key {mpr}{rewrite}[]{\let \mpr@fraction \mpr@@rewrite}
\define@key {mpr}{myfraction}[]{\let \mpr@fraction #1}
\define@key {mpr}{fraction}[]{\def \mpr@fraction {\mpr@make@fraction #1}}
\define@key {mpr}{left}{\setbox0 \hbox {$\TirName {#1}\;$}\relax
     \advance \hsize by -\wd0\box0}
\define@key {mpr}{width}{\hsize #1}
\define@key {mpr}{sep}{\def\mpr@sep{#1}}
\define@key {mpr}{before}{#1}
\define@key {mpr}{lab}{\let \RefTirName \TirName \def \mpr@rulename {#1}}
\define@key {mpr}{Lab}{\let \RefTirName \TirName \def \mpr@rulename {#1}}
\define@key {mpr}{narrower}{\hsize #1\hsize}
\define@key {mpr}{leftskip}{\hskip -#1}
\define@key {mpr}{reduce}[]{\let \mpr@fraction \mpr@@reduce}
\define@key {mpr}{rightskip}
  {\setbox \mpr@right \hbox {\unhbox \mpr@right \hskip -#1}}
\define@key {mpr}{LEFT}{\setbox0 \hbox {$#1$}\relax
     \advance \hsize by -\wd0\box0}
\define@key {mpr}{left}{\setbox0 \hbox {$\TirName {#1}\;$}\relax
     \advance \hsize by -\wd0\box0}
\define@key {mpr}{Left}{\llap{$\TirName {#1}\;$}}
\define@key {mpr}{right}
  {\setbox0 \hbox {$\;\TirName {#1}$}\relax \advance \hsize by -\wd0
   \setbox \mpr@right \hbox {\unhbox \mpr@right \unhbox0}}
\define@key {mpr}{RIGHT}
  {\setbox0 \hbox {$#1$}\relax \advance \hsize by -\wd0
   \setbox \mpr@right \hbox {\unhbox \mpr@right \unhbox0}}
\define@key {mpr}{Right}
  {\setbox \mpr@right \hbox {\unhbox \mpr@right \rlap {$\;\TirName {#1}$}}}
\define@key {mpr}{vdots}{\def \mpr@vdots {\@@atop \mpr@vdotfil{#1}}}
\define@key {mpr}{after}{\edef \mpr@after {\mpr@after #1}}

\newcommand \mpr@inferstar@ [3][]{\setbox0
  \hbox {\let \mpr@rulename \mpr@empty \let \mpr@vdots \relax
         \setbox \mpr@right \hbox{}%
         $\setkeys{mpr}{#1}%
          \ifx \mpr@rulename \mpr@empty \mpr@inferrule {#2}{#3}\else
          \mpr@inferrule [{\mpr@rulename}]{#2}{#3}\fi
          \box \mpr@right \mpr@vdots$}
  \setbox1 \hbox {\strut}
  \@tempdima \dp0 \advance \@tempdima by -\dp1
  \raise \@tempdima \box0}

\def \mpr@infer {\@ifnextchar *{\mpr@inferstar}{\mpr@inferrule}}
\newcommand \mpr@err@skipargs[3][]{}
\def \mpr@inferstar*{\ifmmode 
    \let \@do \mpr@inferstar@
  \else 
    \let \@do \mpr@err@skipargs
    \PackageError {mathpartir}
      {\string\inferrule* can only be used in math mode}{}%
  \fi \@do}


%%% Exports

% Envirnonment mathpar

\let \inferrule \mpr@infer

% make a short name \infer is not already defined
\@ifundefined {infer}{\let \infer \mpr@infer}{}

\def \TirNameStyle #1{\small \textsc{#1}}
\def \tir@name #1{\hbox {\small \TirNameStyle{#1}}}
\let \TirName \tir@name
\let \DefTirName \TirName
\let \RefTirName \TirName

%%% Other Exports

% \let \listcons \mpr@cons
% \let \listsnoc \mpr@snoc
% \let \listhead \mpr@head
% \let \listmake \mpr@makelist




\endinput

